A Macromodeling Approach to Efficiently Compute Scattering from Large Arrays of Complex Scatterers

Full-wave electromagnetic simulations of electrically large arrays of complex antennas and scatterers are challenging, as they consume large amount of memory and require long CPU times. This paper presents a new reduced-order modeling technique to compute scattering and radiation from large arrays of complex scatterers and antennas. In the proposed technique, each element of the array is replaced by an equivalent electric current distribution on a fictitious closed surface enclosing the element. This equivalent electric current density is derived using the equivalence theorem and it is related to the surface currents on the scatterer by the Stratton-Chu formulation. With the proposed approach, instead of directly solving for the unknown surface current density on the scatterers, we only need to solve for the unknowns on the equivalent surface. This approach leads to a reduction in the number of unknowns and better conditioning when it is applied to problems involving complex scatterers with multiscale features. Furthermore, the proposed approach is accelerated with the adaptive integral equation method to solve large problems. As illustrated in several practical examples, the proposed method yields speed up of up to 20 times and consumes up to 12 times less memory than the standard method of moments accelerated with the adaptive integral method.

==> TikzFigure/array_bottom.tex <==

\coordinate (p1) at (-\UnitcellWidth*0.5,-\UnitcellLength*0.5);
\coordinate (p2) at (\UnitcellWidth*0.5,-\UnitcellLength*0.5);
\coordinate (p3) at (\UnitcellWidth*0.5, \UnitcellLength*0.5);
\coordinate (p4) at (-\UnitcellWidth*0.5,\UnitcellLength*0.5);

%%%%%%%%%%%%%MEANDER OUTER STARTS%%%%%%%%%
% Outer loop...
% Top side:
\foreach \x in {1,...,\numgroove}
{	 
  \coordinate (ct1\x) at  ({(-3+\x)*(\ml+2*\mw) - (\ml/2+\mw)} , {2.5*(\ml+2*\mw)+\mw + 0});
  \coordinate (ct2\x) at  ({(-3+\x)*(\ml+2*\mw) - (\ml/4+\mw)} , {2.5*(\ml+2*\mw)+\mw +0});
  \coordinate (ct3\x) at  ({(-3+\x)*(\ml+2*\mw) - (\ml/4+\mw)} , {2.5*(\ml+2*\mw) +\mh});
  \coordinate (ct4\x) at  ({(-3+\x)*(\ml+2*\mw) + (\ml/4+\mw)} , {2.5*(\ml+2*\mw) +\mh});
  \coordinate (ct5\x) at  ({(-3+\x)*(\ml+2*\mw) + (\ml/4+\mw)} , {2.5*(\ml+2*\mw)+\mw +0});
  \coordinate (ct6\x) at  ({(-3+\x)*(\ml+2*\mw) + (\ml/2+\mw)} , {2.5*(\ml+2*\mw)+\mw +0});

%			\coordinate (c2\x) at  ({2*\meanderw*\x}, \meanderh );
%			\coordinate (c3\x) at  ({2*\meanderw*\x + \meanderw}, \meanderh );
%	  \coordinate (c4\x) at  ({2*\meanderw*\x + \meanderw}, 0 );
}


\coordinate (ccornertr) at ({2.5*(\ml+2*\mw) + \mw}, {2.5*(\ml+2*\mw) + \mw});

% Outer loop
% right side
\foreach \x in {1,...,\numgroove}
{	 
  \coordinate (cr1\x) at  ({2.5*(\ml+2*\mw)+\mw + 0},     {(3-\x)*(\ml+2*\mw) + (\ml/2+\mw)});
  \coordinate (cr2\x) at  ( {2.5*(\ml+2*\mw)+\mw +0}, {(3-\x)*(\ml+2*\mw) + (\ml/4+\mw)});
  \coordinate (cr3\x) at  ({2.5*(\ml+2*\mw) +\mh}, {(3-\x)*(\ml+2*\mw) + (\ml/4+\mw)} );
  \coordinate (cr4\x) at  ({2.5*(\ml+2*\mw) +\mh}, {(3-\x)*(\ml+2*\mw) - (\ml/4+\mw)} );
  \coordinate (cr5\x) at  ({2.5*(\ml+2*\mw)+\mw +0}, {(3-\x)*(\ml+2*\mw) - (\ml/4+\mw)} );
  \coordinate (cr6\x) at  ({2.5*(\ml+2*\mw)+\mw +0}, {(3-\x)*(\ml+2*\mw) - (\ml/2+\mw)} );
%			\coordinate (c2\x) at  ({2*\meanderw*\x}, \meanderh );
%			\coordinate (c3\x) at  ({2*\meanderw*\x + \meanderw}, \meanderh );
%	  \coordinate (c4\x) at  ({2*\meanderw*\x + \meanderw}, 0 );
}
\coordinate (ccornerbr) at ({2.5*(\ml+2*\mw) + \mw}, {-2.5*(\ml+2*\mw) - \mw});




% Outer loop
% bottom side
\foreach \x in {1,...,\numgroove}
{	 
  \coordinate (cb1\x) at  ({(3-\x)*(\ml+2*\mw) + (\ml/2+\mw)}, {-2.5*(\ml+2*\mw)-\mw + 0});
  \coordinate (cb2\x) at  ({(3-\x)*(\ml+2*\mw) + (\ml/4+\mw)}, {-2.5*(\ml+2*\mw)-\mw + 0});
  \coordinate (cb3\x) at  ({(3-\x)*(\ml+2*\mw) + (\ml/4+\mw)}, {-2.5*(\ml+2*\mw)-\mh});
  \coordinate (cb4\x) at  ({(3-\x)*(\ml+2*\mw) - (\ml/4+\mw)}, {-2.5*(\ml+2*\mw)-\mh});
  \coordinate (cb5\x) at  ({(3-\x)*(\ml+2*\mw) - (\ml/4+\mw)}, {-2.5*(\ml+2*\mw)-\mw});
  \coordinate (cb6\x) at  ({(3-\x)*(\ml+2*\mw) - (\ml/2+\mw)}, {-2.5*(\ml+2*\mw)-\mw});
%			\coordinate (c2\x) at  ({2*\meanderw*\x}, \meanderh );
%			\coordinate (c3\x) at  ({2*\meanderw*\x + \meanderw}, \meanderh );
%	  \coordinate (c4\x) at  ({2*\meanderw*\x + \meanderw}, 0 );
}

\coordinate (ccornerbl) at ({-2.5*(\ml+2*\mw) - \mw}, {-2.5*(\ml+2*\mw) - \mw});

% Outer loop
% left side
\foreach \x in {1,...,\numgroove}
{	 
  \coordinate (cl1\x) at  ({-2.5*(\ml+2*\mw)-\mw + 0}, {(-3+\x)*(\ml+2*\mw) - (\ml/2+\mw)});
    \coordinate (cl2\x) at  ({-2.5*(\ml+2*\mw)-\mw + 0}, {(-3+\x)*(\ml+2*\mw) - (\ml/4+\mw)});
     \coordinate (cl3\x) at  ({-2.5*(\ml+2*\mw)-\mh + 0}, {(-3+\x)*(\ml+2*\mw) - (\ml/4+\mw)});
     \coordinate (cl4\x) at  ({-2.5*(\ml+2*\mw)-\mh + 0}, {(-3+\x)*(\ml+2*\mw) + (\ml/4+\mw)});
     \coordinate (cl5\x) at  ({-2.5*(\ml+2*\mw)-\mw + 0}, {(-3+\x)*(\ml+2*\mw) + (\ml/4+\mw)});
     \coordinate (cl6\x) at  ({-2.5*(\ml+2*\mw)-\mw + 0}, {(-3+\x)*(\ml+2*\mw) + (\ml/2+\mw)});
     
%			\coordinate (c2\x) at  ({2*\meanderw*\x}, \meanderh );
%			\coordinate (c3\x) at  ({2*\meanderw*\x + \meanderw}, \meanderh );
%	  \coordinate (c4\x) at  ({2*\meanderw*\x + \meanderw}, 0 );
}

\coordinate (ccornertl) at ({-2.5*(\ml+2*\mw) - \mw}, {2.5*(\ml+2*\mw) + \mw});


%%%%%%%%%%%%%MEANDER OUTER ENDS%%%%%%%%%








%%%%%%%%%%%%%MEANDER INNER STARTS%%%%%%%%%
% Outer loop...
% Top side:
\foreach \x in {1,...,\numgroove}
{	 
  \coordinate (inct1\x) at  ({(-3+\x)*(\ml+2*\mw) - (\ml/2+\mw)} , {2.5*(\ml+2*\mw) + 0});
  \coordinate (inct2\x) at  ({(-3+\x)*(\ml+2*\mw) - (\ml/4)} , {2.5*(\ml+2*\mw) +0});
  \coordinate (inct3\x) at  ({(-3+\x)*(\ml+2*\mw) - (\ml/4)} , {2.5*(\ml+2*\mw) +\mh - \mw});
  \coordinate (inct4\x) at  ({(-3+\x)*(\ml+2*\mw) + (\ml/4)} , {2.5*(\ml+2*\mw) +\mh - \mw});
  \coordinate (inct5\x) at  ({(-3+\x)*(\ml+2*\mw) + (\ml/4)} , {2.5*(\ml+2*\mw) +0});
  \coordinate (inct6\x) at  ({(-3+\x)*(\ml+2*\mw) + (\ml/2+\mw)} , {2.5*(\ml+2*\mw) +0});

%			\coordinate (c2\x) at  ({2*\meanderw*\x}, \meanderh );
%			\coordinate (c3\x) at  ({2*\meanderw*\x + \meanderw}, \meanderh );
%	  \coordinate (c4\x) at  ({2*\meanderw*\x + \meanderw}, 0 );
}


\coordinate (inccornertr) at ({2.5*(\ml+2*\mw) }, {2.5*(\ml+2*\mw) });

% Outer loop
% right side
\foreach \x in {1,...,\numgroove}
{	 
  \coordinate (incr1\x) at  ({2.5*(\ml+2*\mw) + 0},     {(3-\x)*(\ml+2*\mw) + (\ml/2+\mw)});
  \coordinate (incr2\x) at  ( {2.5*(\ml+2*\mw) +0}, {(3-\x)*(\ml+2*\mw) + (\ml/4)});
  \coordinate (incr3\x) at  ({2.5*(\ml+2*\mw) +\mh - \mw}, {(3-\x)*(\ml+2*\mw) + (\ml/4)} );
  \coordinate (incr4\x) at  ({2.5*(\ml+2*\mw) +\mh - \mw}, {(3-\x)*(\ml+2*\mw) - (\ml/4)} );
  \coordinate (incr5\x) at  ({2.5*(\ml+2*\mw) +0}, {(3-\x)*(\ml+2*\mw) - (\ml/4)} );
  \coordinate (incr6\x) at  ({2.5*(\ml+2*\mw) +0}, {(3-\x)*(\ml+2*\mw) - (\ml/2+\mw)} );
%			\coordinate (c2\x) at  ({2*\meanderw*\x}, \meanderh );
%			\coordinate (c3\x) at  ({2*\meanderw*\x + \meanderw}, \meanderh );
%	  \coordinate (c4\x) at  ({2*\meanderw*\x + \meanderw}, 0 );
}
\coordinate (inccornerbr) at ({2.5*(\ml+2*\mw) }, {-2.5*(\ml+2*\mw) });




% Outer loop
% bottom side
\foreach \x in {1,...,\numgroove}
{	 
  \coordinate (incb1\x) at  ({(3-\x)*(\ml+2*\mw) + (\ml/2+\mw)}, {-2.5*(\ml+2*\mw)- 0});
  \coordinate (incb2\x) at  ({(3-\x)*(\ml+2*\mw) + (\ml/4)}, {-2.5*(\ml+2*\mw)- 0});
  \coordinate (incb3\x) at  ({(3-\x)*(\ml+2*\mw) + (\ml/4)}, {-2.5*(\ml+2*\mw)-\mh + \mw});
  \coordinate (incb4\x) at  ({(3-\x)*(\ml+2*\mw) - (\ml/4)}, {-2.5*(\ml+2*\mw)-\mh + \mw});
  \coordinate (incb5\x) at  ({(3-\x)*(\ml+2*\mw) - (\ml/4)}, {-2.5*(\ml+2*\mw)});
  \coordinate (incb6\x) at  ({(3-\x)*(\ml+2*\mw) - (\ml/2+\mw)}, {-2.5*(\ml+2*\mw)});
%			\coordinate (c2\x) at  ({2*\meanderw*\x}, \meanderh );
%			\coordinate (c3\x) at  ({2*\meanderw*\x + \meanderw}, \meanderh );
%	  \coordinate (c4\x) at  ({2*\meanderw*\x + \meanderw}, 0 );
}

\coordinate (inccornerbl) at ({-2.5*(\ml+2*\mw) }, {-2.5*(\ml+2*\mw) });

% Outer loop
% left side
\foreach \x in {1,...,\numgroove}
{	 
  \coordinate (incl1\x) at  ({-2.5*(\ml+2*\mw)+ 0}, {(-3+\x)*(\ml+2*\mw) - (\ml/2+\mw)});
    \coordinate (incl2\x) at  ({-2.5*(\ml+2*\mw) + 0}, {(-3+\x)*(\ml+2*\mw) - (\ml/4)});
     \coordinate (incl3\x) at  ({-2.5*(\ml+2*\mw)-\mh+\mw + 0}, {(-3+\x)*(\ml+2*\mw) - (\ml/4)});
     \coordinate (incl4\x) at  ({-2.5*(\ml+2*\mw)-\mh + \mw+ 0}, {(-3+\x)*(\ml+2*\mw) + (\ml/4)});
     \coordinate (incl5\x) at  ({-2.5*(\ml+2*\mw) + 0}, {(-3+\x)*(\ml+2*\mw) + (\ml/4)});
     \coordinate (incl6\x) at  ({-2.5*(\ml+2*\mw) + 0}, {(-3+\x)*(\ml+2*\mw) + (\ml/2+\mw)});
     
%			\coordinate (c2\x) at  ({2*\meanderw*\x}, \meanderh );
%			\coordinate (c3\x) at  ({2*\meanderw*\x + \meanderw}, \meanderh );
%	  \coordinate (c4\x) at  ({2*\meanderw*\x + \meanderw}, 0 );
}

\coordinate (inccornertl) at ({-2.5*(\ml+2*\mw)}, {2.5*(\ml+2*\mw)});


\draw[fill = brown!90]  (ct11) -- (ct21) -- (ct31) -- (ct41) -- (ct51) -- (ct61)--
(ct12) -- (ct22) -- (ct32) -- (ct42) -- (ct52) --(ct62)--
(ct13) -- (ct23) -- (ct33) --  (ct43) -- (ct53) --(ct63)--
(ct14) -- (ct24) -- (ct34)-- (ct44) -- (ct54) --(ct64)--
(ct15) -- (ct25) -- (ct35) -- (ct45) -- (ct55) -- (ct65)--
(ccornertr) --
(cr11) -- (cr21) -- (cr31) -- (cr41) -- (cr51) -- (cr61) --
(cr12) -- (cr22) -- (cr32) -- (cr42) -- (cr52) -- (cr62) --
(cr13) -- (cr23) -- (cr33) -- (cr43) -- (cr53) -- (cr63) --
(cr14) -- (cr24) -- (cr34) -- (cr44) -- (cr54) -- (cr64) --
(cr15) -- (cr25) -- (cr35) -- (cr45) -- (cr55) -- (cr65) --
(ccornerbr) --
(cb11) -- (cb21) -- (cb31)-- (cb41) -- (cb51) -- (cb61) --
(cb12) -- (cb22) --(cb32)-- (cb42) -- (cb52) -- (cb62) --
(cb13) -- (cb23) --(cb33)--(cb43) -- (cb53) -- (cb63) --
(cb14) -- (cb24) --(cb34)--(cb44) -- (cb54) -- (cb64) --
(cb15) -- (cb25) --(cb35)-- (cb45) -- (cb55) -- (cb65) --
(ccornerbl) --
(cl11) -- (cl21) -- (cl31) -- (cl41) -- (cl51) -- (cl61) --
(cl12) -- (cl22) -- (cl32) -- (cl42) -- (cl52) -- (cl62) --
(cl13) -- (cl23) -- (cl33) -- (cl43) -- (cl53) -- (cl63) --
(cl14) -- (cl24) -- (cl34) -- (cl44) -- (cl54) -- (cl64) --
(cl15) -- (cl25) -- (cl35) -- (cl45) -- (cl55) -- (cl65) --
(ccornertl) -- (ct11) -- 
(inct11) -- (inccornertl) --
(incl65) -- (incl55) -- (incl45) -- (incl35) -- (incl25) -- (incl15) --
(incl64) -- (incl54) -- (incl44) -- (incl34) -- (incl24) -- (incl14) --
(incl63) -- (incl53) -- (incl43) -- (incl33) -- (incl23) -- (incl13) --
(incl62) -- (incl52) -- (incl42) -- (incl32) -- (incl22) -- (incl12) --
(incl61) -- (incl51) -- (incl41) -- (incl31) -- (incl21) -- (incl11) --
(inccornerbl) --
(incb65) -- (incb55) --(incb45)-- (incb35) -- (incb25) -- (incb15) --
(incb64) -- (incb54) --(incb44)--(incb34) -- (incb24) -- (incb14) --
(incb63) -- (incb53) --(incb43)--(incb33) -- (incb23) -- (incb13) --
(incb62) -- (incb52) --(incb42)-- (incb32) -- (incb22) -- (incb12) --
(incb61) -- (incb51) -- (incb41)-- (incb31) -- (incb21) -- (incb11) --
(inccornerbr) --
(incr65) -- (incr55) -- (incr45) -- (incr35) -- (incr25) -- (incr15) --
(incr64) -- (incr54) -- (incr44) -- (incr34) -- (incr24) -- (incr14) --
(incr63) -- (incr53) -- (incr43) -- (incr33) -- (incr23) -- (incr13) --
(incr62) -- (incr52) -- (incr42) -- (incr32) -- (incr22) -- (incr12) --
(incr61) -- (incr51) -- (incr41) -- (incr31) -- (incr21) -- (incr11) --
(inccornertr) --
(inct65) -- (inct55) -- (inct45) -- (inct35) -- (inct25) -- (inct15)--
(inct64) -- (inct54) -- (inct44)-- (inct34) -- (inct24) --(inct14)--
(inct63) -- (inct53) -- (inct43) --  (inct33) -- (inct23) --(inct13)--
(inct62) -- (inct52) -- (inct42) -- (inct32) -- (inct22) --(inct12)--
(inct61) -- (inct51) -- (inct41) -- (inct31) -- (inct21) -- (inct11)--
(ct11);







%\draw[fill = white] 






%%%%%%%%%%%%%MEANDER INNER ENDS%%%%%%%%%


%%%%%%%%%%%%% INNER LOOP %%%%%%%%%%%%%
\coordinate (c1o) at ({-\InnerLoopWout/2}, {-\InnerLoopWout/2});
\coordinate (c2o) at ({-\InnerLoopWout/2}, {\InnerLoopWout/2});
\coordinate (c3o) at ({\InnerLoopWout/2}, {\InnerLoopWout/2});
\coordinate (c4o) at ({\InnerLoopWout/2}, {-\InnerLoopWout/2});

\coordinate (c1op) at ({-\InnerLoopWout/2 + \epsthres}, {-\InnerLoopWout/2});
%\draw [fill = brown!70] (c1) -- (c2) -- (c3) -- (c4) -- (c1);

\coordinate (c1ip) at ({-\InnerLoopWin/2 + \epsthres}, {-\InnerLoopWin/2});

\coordinate (c1i) at ({-\InnerLoopWin/2}, {-\InnerLoopWin/2});
\coordinate (c2i) at ({-\InnerLoopWin/2}, {\InnerLoopWin/2});
\coordinate (c3i) at ({\InnerLoopWin/2}, {\InnerLoopWin/2});
\coordinate (c4i) at ({\InnerLoopWin/2}, {-\InnerLoopWin/2});


==> TikzFigure/array_middle.tex <==
\foreach \x in {1,...,\numgroove}
{	 
  \coordinate (t1\x) at  ({(-2+\x)*(\ml+2*\mw) - (\ml/2+\mw)} , {0.5*\ldyl});
  \coordinate (t2\x) at  ({(-2+\x)*(\ml+2*\mw) - (\ml/4)} , {0.5*\ldyl});
  \coordinate (t3\x) at  ({(-2+\x)*(\ml+2*\mw) - (\ml/4)} , {0.5*\ldyl +\mh});
  \coordinate (t4\x) at  ({(-2+\x)*(\ml+2*\mw) + (\ml/4)} , {0.5*\ldyl +\mh});
  \coordinate (t5\x) at  ({(-2+\x)*(\ml+2*\mw) + (\ml/4)} , {0.5*\ldyl +0});
  \coordinate (t6\x) at  ({(-2+\x)*(\ml+2*\mw) + (\ml/2+\mw)} , {0.5*\ldyl +0});
}



% right side
\foreach \x in {1,...,\numgroove}
{	 
  \coordinate (r1\x) at  ({\ldxl*0.5 + 0},     {(2-\x)*(\ml+2*\mw) + (\ml/2+\mw) });
  \coordinate (r2\x) at  ( {\ldxl*0.5 +0}, {(2-\x)*(\ml+2*\mw) + (\ml/4+\mw)});
  \coordinate (r3\x) at  ({\ldxl*0.5 +\mh}, {(2-\x)*(\ml+2*\mw) +(\ml/4+\mw)} );
  \coordinate (r4\x) at  ({\ldxl*0.5 +\mh}, {(2-\x)*(\ml+2*\mw) - (\ml/4+\mw)} );
  \coordinate (r5\x) at  ({\ldxl*0.5 +0}, {(2-\x)*(\ml+2*\mw)  - (\ml/4+\mw)} );
  \coordinate (r6\x) at  ({\ldxl*0.5+0}, {(2-\x)*(\ml+2*\mw)- (\ml/2+\mw) } );
}

% bottom side
\foreach \x in {1,...,\numgroove}
{	 
  \coordinate (b1\x) at  ({(2-\x)*(\ml+2*\mw) + (\ml/2+\mw)}, {-{0.5*\ldyl}- 0});
  \coordinate (b2\x) at  ({(2-\x)*(\ml+2*\mw) + (\ml/4)}, {-{0.5*\ldyl}- 0});
  \coordinate (b3\x) at  ({(2-\x)*(\ml+2*\mw) + (\ml/4)}, {-{0.5*\ldyl}-\mh });
  \coordinate (b4\x) at  ({(2-\x)*(\ml+2*\mw) - (\ml/4)}, {-{0.5*\ldyl}-\mh});
  \coordinate (b5\x) at  ({(2-\x)*(\ml+2*\mw) - (\ml/4)}, {-{0.5*\ldyl}});
  \coordinate (b6\x) at  ({(2-\x)*(\ml+2*\mw) - (\ml/2+\mw)}, {-{0.5*\ldyl}});

}

% left side
\foreach \x in {1,...,\numgroove}
{	 
  \coordinate (l1\x) at  ({-\ldxl*0.5+ 0}, {(-2+\x)*(\ml+2*\mw) - (\ml/2+\mw)});
    \coordinate (l2\x) at  ({-\ldxl*0.5 + 0}, {(-2+\x)*(\ml+2*\mw) - (\ml/4)});
     \coordinate (l3\x) at  ({-\ldxl*0.5-\mh + 0}, {(-2+\x)*(\ml+2*\mw) - (\ml/4)});
     \coordinate (l4\x) at  ({-\ldxl*0.5-\mh }, {(-2+\x)*(\ml+2*\mw) + (\ml/4)});
     \coordinate (l5\x) at  ({-\ldxl*0.5}, {(-2+\x)*(\ml+2*\mw) + (\ml/4)});
     \coordinate (l6\x) at  ({-\ldxl*0.5}, {(-2+\x)*(\ml+2*\mw) + (\ml/2+\mw)});
     
}


\draw (l11) -- (l21) -- (l31) -- (l41) -- (l51) -- (l61) --
(l12) -- (l22) -- (l32) -- (l42) -- (l52) -- (l62) -- 
(l13) -- (l23) -- (l33) -- (l43) -- (l53) -- (l63);

\coordinate (pp+1) at ($(-0.5*\lcxl, 0.5*\ldyl )$);
\coordinate (pp+2) at ($(\lcxl*0.5, \ldyl*0.5)$);
\coordinate (pp+3) at ($(\lcxl*0.5, \ldyl*0.5 - \wcyl)$);
\coordinate (pp+4) at ($(\wdxl*0.5, \ldyl*0.5 - \wcyl)$);
\coordinate (pp+5) at ($(\wdxl*0.5, \wdyl*0.5)$);
\coordinate (pp+6) at ($(\ldxl*0.5 - \wcxl, \wdyl*0.5)$);
\coordinate (pp+7) at ($(\ldxl*0.5 - \wcxl, \lcyl*0.5)$);
\coordinate (pp+8) at ($(\ldxl*0.5, \lcyl*0.5)$);
\coordinate (pp+9) at ($(\ldxl*0.5, -\lcyl*0.5)$);
\coordinate (pp+10) at ($(\ldxl*0.5- \wcxl, -\lcyl*0.5)$);
\coordinate (pp+11) at ($(\ldxl*0.5 - \wcxl,  -\wdyl*0.5)$);
\coordinate (pp+12) at ($(\wdxl*0.5, -\wdyl*0.5)$);
\coordinate (pp+13) at ($(\wdxl*0.5, -\ldyl*0.5 + \wcyl)$);
\coordinate (pp+14) at ($(\lcxl*0.5,  -\ldyl*0.5 + \wcyl)$);
\coordinate (pp+15) at ($(\lcxl*0.5, -\ldyl*0.5)$);
\coordinate (pp+16) at ($(-\lcxl*0.5, -\ldyl*0.5)$);
\coordinate (pp+17) at ($(-\lcxl*0.5, -\ldyl*0.5+ \wcyl)$);
\coordinate (pp+18) at ($(-\wdxl*0.5, -\ldyl*0.5+\wcyl)$);
\coordinate (pp+19) at ($(-\wdxl*0.5,  -\wdyl*0.5)$);
\coordinate (pp+20) at ($(-\ldxl*0.5 + \wcxl, -\wdyl*0.5)$);
\coordinate (pp+21) at ($(-\ldxl*0.5 + \wcxl,  -\lcyl*0.5)$);
\coordinate (pp+22) at ($(-\ldxl*0.5,  -\lcyl*0.5)$);
\coordinate (pp+23) at ($(-\ldxl*0.5, \lcyl*0.5)$);
\coordinate (pp+24) at ($(-\ldxl*0.5+\wcxl, \lcyl*0.5)$);
\coordinate (pp+25) at ($(-\ldxl*0.5+\wcxl,  \wdyl*0.5)$);
\coordinate (pp+26) at ($(-\wdxl*0.5,  \wdyl*0.5)$);
\coordinate (pp+27) at ($(-\wdxl*0.5,  \ldyl*0.5-\wcyl)$);
\coordinate (pp+28) at ($(-\lcxl*0.5,  \ldyl*0.5-\wcyl)$);

\draw (t11) -- (t21) -- (t31) -- (t41) -- (t51) -- (t61) --
(t12) -- (t22) -- (t32) -- (t42) -- (t52) -- (t62) --
(t13) -- (t23) -- (t33) -- (t43) -- (t53) -- (t63);

\draw[fill = brown!90] (pp+1) -- (t11) -- (t21) -- (t31) -- (t41) -- (t51) -- (t61) --
(t12) -- (t22) -- (t32) -- (t42) -- (t52) -- (t62) --
(t13) -- (t23) -- (t33) -- (t43) -- (t53) -- (t63) --
(pp+2) -- (pp+3) -- (pp+4) -- (pp+5) -- (pp+6) -- (pp+7) -- (pp+8) -- 
(r11) -- (r21) -- (r31) -- (r41) -- (r51) -- (r61)
-- (r12) -- (r22) -- (r32) -- (r42) -- (r52) -- (r62) --
(r13) -- (r23) -- (r33) -- (r43) -- (r53) -- (r63) --
(pp+9) --(pp+10) --(pp+11) --(pp+12) --(pp+13) --(pp+14) --(pp+15) --
(b11) -- (b21) -- (b31) -- (b41) -- (b51) -- (b61) -- (b12) -- (b22) -- (b32) -- (b42) -- (b52) -- (b62) --
(b13) -- (b23) -- (b33) -- (b43) -- (b53) -- (b63) --
(pp+16) --(pp+17) --(pp+18) --(pp+19) --(pp+20) --(pp+21) --(pp+22) --(pp+22) --
(l11) -- (l21) -- (l31) -- (l41) -- (l51) -- (l61) --
(l12) -- (l22) -- (l32) -- (l42) -- (l52) -- (l62) -- 
(l13) -- (l23) -- (l33) -- (l43) -- (l53) -- (l63) --
(pp+23) --(pp+24) --(pp+25) --(pp+26) --(pp+27) --(pp+28) --(pp+1);

